Non-standard approximations of the Ito-map

The Wong-Zakai theorem asserts that ODEs driven by "reasonable" (e.g. piecewise linear) approximations of Brownian motion converge to the corresponding Stratonovich stochastic differential equation. With the aid of rough path analysis, we study "non-reasonable" approximations and go beyond a well-known criterion of [Ikeda--Watanabe, North Holland 1989] in the sense that our result applies to perturbations on all levels, exhibiting additional drift terms involving any iterated Lie brackets of the driving vector fields. In particular, this applies to the approximations by McShane ('72) and Sussmann ('91). Our approach is not restricted to Brownian driving signals. At last, these ideas can be used to prove optimality of certain rough path estimates.

==> apreambl.tex <==
% This is APREAMBL.TEX, version 1.10e, written by Hans-Hermann Bode
% (HHBODE@DOSUNI1.BITNET), for the BibTeX `adaptable' family, version 1.10.
% See the file APREAMBL.DOC for a detailed documentation.

% This program is distributed WITHOUT ANY WARRANTY, express or implied.

% Copyright (C) 1991, 1992 Hans-Hermann Bode

% Permission is granted to make and distribute verbatim copies of this
% document provided that the copyright notice and this permission notice
% are preserved on all copies.

% Permission is granted to copy and distribute modified versions of this
% document under the conditions for verbatim copying, provided that the
% entire resulting derived work is distributed under the terms of a
% permission notice identical to this one.
\expandafter\ifx\csname__APREAMBLE_TEX\endcsname\relax \else\endinput\fi
\expandafter\chardef\csname__APREAMBLE_TEX\endcsname=\the\catcode`\@
\catcode`\@=11
\gdef\abtype@english{%
\def\abtype##1##2{%
\ifcase##1{\sc##2}\or``##2''\or{\em##2\/}\or{\bf##2}\or(##2)\or(##2)\else##2\fi}}

\gdef\abtype@german{%
\def\abtype##1##2{%
\ifcase##1{\sc##2}\or\glqq##2\grqq\or{\em##2\/}\or{\bf##2}\or(##2)\or(##2)\else##2\fi}}
\ifabfull

\gdef\abetc@english{

\def\abphrase##1{%
\ifcase##1{ and }\or{,}\or{ et~al.}\or{, editors}\or{, editor}\or%
{ of }\or{ in }\or{In }\or{volume}\or{Volume}\or{number}\or{Number}\or%
{ edition}\or{pages}\or{page}\or{chapter}\or%
{Technical Report}\or{Master's thesis}\or{PhD thesis}\fi}

\def\abmonth##1{\ifcase##1\or January\or February\or March\or April\or May\or
  June\or July\or August\or September\or October\or November\or December\fi}

\def\abedition##1{\ifcase##1\or First\or Second\or Third\or Fourth\or Fifth\or
  Sixth\or Seventh\or Eighth\or Ninth\or Tenth\else?\fi}

\def\abchapter##1{\ifcase##1Section\or Paragraph\or Appendix\or Part\fi}

}

\else

\gdef\abetc@english{

\def\abphrase##1{%
\ifcase##1{ and }\or{,}\or{ et~al.}\or{, editors}\or{, editor}\or%
{ of }\or{ in }\or{In }\or{vol.}\or{Vol.}\or{no.}\or{No.}\or%
{ ed.}\or{pp.}\or{p.}\or{ch.}\or%
{Technical Report}\or{Master's thesis}\or{PhD thesis}\fi}

\def\abmonth##1{\ifcase##1\or Jan.\or Feb.\or Mar.\or Apr.\or May\or June\or
  July\or Aug.\or Sept.\or Oct.\or Nov.\or Dec.\fi}

\def\abedition##1{\ifcase##1\or 1st\or 2nd\or 3rd\or 4th\or 5th\or
  6th\or 7th\or 8th\or 9th\or 10th\else?\fi}

\def\abchapter##1{\ifcase##1Sec.\or Par.\or App.\or Part\fi}

}

\fi
\ifabfull

\gdef\abetc@german{

\def\abphrase##1{%
\ifcase##1{ und }\or{}\or{ und andere}\or{ (Herausgeber)}\or{ (Herausgeber)}\or%
{ aus }\or{ in }\or{In }\or{Band}\or{Band}\or{Nummer}\or{Nummer}\or%
{ Auf{\kern0pt}lage}\or{Seiten}\or{Seite}\or{Kapitel}\or%
{Bericht}\or{Diplomarbeit}\or{Dissertation}\fi}

\def\abmonth##1{\ifcase##1\or Januar\or Februar\or M\"arz\or April\or Mai\or
  Juni\or Juli\or August\or September\or Oktober\or November\or Dezember\fi}

\def\abedition##1{\ifcase##1\or Erste\or Zweite\or Dritte\or Vierte\or F\"unf\-te\or
  Sechste\or Siebte\or Achte\or Neunte\or Zehnte\else?\fi}

\def\abchapter##1{\ifcase##1Abschnitt\or Absatz\or Anhang\or Teil\fi}

}

\else

\gdef\abetc@german{

\def\abphrase##1{%
\ifcase##1{ und }\or{}\or{ u.\thinspace a.}\or{ (Hrsg.)}\or{ (Hrsg.)}\or%
{ aus }\or{ in }\or{In }\or{Bd.}\or{Bd.}\or{Nr.}\or{Nr.}\or%
{ Aufl.}\or{S.}\or{S.}\or{Kap.}\or%
{Bericht}\or{Diplomarbeit}\or{Dissertation}\fi}

\def\abmonth##1{\ifcase##1\or Jan.\or Feb.\or M\"arz\or Apr.\or Mai\or
  Juni\or Juli\or Aug.\or Sep.\or Okt.\or Nov.\or Dez.\fi}

\def\abedition##1{\ifcase##1\or 1.\or 2.\or 3.\or 4.\or 5.\or
  6.\or 7.\or 8.\or 9.\or 10.\else?\fi}

\def\abchapter##1{\ifcase##1Abschn.\or Abs.\or Anh.\or Teil\fi}

}

\fi
\expandafter\ifx\csname language\endcsname\relax % \ifundefined{language}
  \csname newcount\endcsname\language
\fi
\expandafter\ifx\csname mdqon\endcsname\relax % \ifundefined{mdqon}
  \chardef\USenglish=0
  \chardef\german=1
  \chardef\austrian=1
  \chardef\french=2
  \chardef\english=0
  \language\USenglish
\else
  \expandafter\ifx\csname l@USenglish\endcsname\relax \else
    \chardef\USenglish=\l@USenglish\fi
  \expandafter\ifx\csname l@german\endcsname\relax \else
    \chardef\german=\l@german\fi
  \expandafter\ifx\csname l@austrian\endcsname\relax \else
    \chardef\austrian=\l@austrian\fi
  \expandafter\ifx\csname l@french\endcsname\relax \else
    \chardef\french=\l@french\fi
  \expandafter\ifx\csname l@english\endcsname\relax \else
    \chardef\english=\l@english\fi
\fi
\ifnum\language=\german
  \abtype@german \abetc@german
\else\ifnum\language=\austrian
  \abtype@german \abetc@german
\else
  \abtype@english \abetc@english
\fi\fi
\catcode`\@=\csname__APREAMBLE_TEX\endcsname
\endinput

